Predictions for Muon Electric and Magnetic Dipole Moments from $h \rightarrow \mu^+ \mu^-$ in Two-Higgs-Doublet Models with New Leptons

We calculate chirally enhanced corrections to the muon's electric and magnetic dipole moments in two-Higgs-doublet models extended by vector-like leptons, and we explore a sharp correlation between $h \rightarrow \mu^+ \mu^-$ and the muon's dipole moments in these models. Among many detailed predictions, for a model with new leptons with the same quantum numbers as standard model leptons, we find that $0.38 \lesssim \tan \beta \lesssim 21$ necessarily requires a muon electric dipole moment to be observed at near-future experiments, assuming $h \rightarrow \mu^+ \mu^-$ is measured within $1\%$ of the standard model prediction for the current central value of the measured muon magnetic moment. In all studied models, the predicted values of the electric dipole moment can reach up to current experimental limits. Moreover, we show that in some models there can be two sources of chiral enhancement, parametrizing the correlation between $h \rightarrow \mu^+ \mu^-$ and the dipole moments by a complex number. This leads to sign-preferred predictions for the electric dipole moment.

==> main-references.tex <==
%\cite{ATLAS:2020fzp}
\bibitem{ATLAS:2020fzp}
G.~Aad \textit{et al.} [ATLAS],
%``A search for the dimuon decay of the Standard Model Higgs boson with the ATLAS detector,''
Phys. Lett. B \textbf{812}, 135980 (2021)
doi:10.1016/j.physletb.2020.135980
[arXiv:2007.07830 [hep-ex]].
%199 citations counted in INSPIRE as of 15 Aug 2023

%\cite{Muong-2:2023cdq}
\bibitem{Muong-2:2023cdq}
D.~P.~Aguillard \textit{et al.} [Muon g-2],
%``Measurement of the Positive Muon Anomalous Magnetic Moment to 0.20 ppm,''
[arXiv:2308.06230 [hep-ex]].
%7 citations counted in INSPIRE as of 21 Aug 2023

%\cite{Aoyama:2020ynm}
\bibitem{Aoyama:2020ynm}
T.~Aoyama, N.~Asmussen, M.~Benayoun, J.~Bijnens, T.~Blum, M.~Bruno, I.~Caprini, C.~M.~Carloni Calame, M.~C\`e and G.~Colangelo, \textit{et al.}
%``The anomalous magnetic moment of the muon in the Standard Model,''
Phys. Rept. \textbf{887}, 1-166 (2020)
doi:10.1016/j.physrep.2020.07.006
[arXiv:2006.04822 [hep-ph]].
%1057 citations counted in INSPIRE as of 21 Aug 2023

%\cite{Borsanyi:2020mff}
\bibitem{Borsanyi:2020mff}
S.~Borsanyi, Z.~Fodor, J.~N.~Guenther, C.~Hoelbling, S.~D.~Katz, L.~Lellouch, T.~Lippert, K.~Miura, L.~Parato and K.~K.~Szabo, \textit{et al.}
%``Leading hadronic contribution to the muon magnetic moment from lattice QCD,''
Nature \textbf{593}, no.7857, 51-55 (2021)
doi:10.1038/s41586-021-03418-1
[arXiv:2002.12347 [hep-lat]].
%657 citations counted in INSPIRE as of 21 Aug 2023

%\cite{CMD-3:2023alj}
\bibitem{CMD-3:2023alj}
F.~V.~Ignatov \textit{et al.} [CMD-3],
%``Measurement of the $e^+e^-\to\pi^+\pi^-$ cross section from threshold to 1.2 GeV with the CMD-3 detector,''
[arXiv:2302.08834 [hep-ex]].
%42 citations counted in INSPIRE as of 21 Aug 2023

%\cite{Fukuyama:2012np}
\bibitem{Fukuyama:2012np}
T.~Fukuyama,
%``Searching for New Physics beyond the Standard Model in Electric Dipole Moment,''
Int. J. Mod. Phys. A \textbf{27}, 1230015 (2012)
doi:10.1142/S0217751X12300153
[arXiv:1201.4252 [hep-ph]].
%133 citations counted in INSPIRE as of 07 Jul 2023

%\cite{Kannike:2011ng}
\bibitem{Kannike:2011ng}
K.~Kannike, M.~Raidal, D.~M.~Straub and A.~Strumia,
%``Anthropic solution to the magnetic muon anomaly: the charged see-saw,''
JHEP \textbf{02}, 106 (2012)
[erratum: JHEP \textbf{10}, 136 (2012)]
doi:10.1007/JHEP02(2012)106
[arXiv:1111.2551 [hep-ph]].
%109 citations counted in INSPIRE as of 16 Aug 2023

%\cite{Dermisek:2013gta}
\bibitem{Dermisek:2013gta}
R.~Dermisek and A.~Raval,
%``Explanation of the Muon g-2 Anomaly with Vectorlike Leptons and its Implications for Higgs Decays,''
Phys. Rev. D \textbf{88}, 013017 (2013)
doi:10.1103/PhysRevD.88.013017
[arXiv:1305.3522 [hep-ph]].
%148 citations counted in INSPIRE as of 16 Aug 2023

%\cite{Crivellin:2021rbq}
\bibitem{Crivellin:2021rbq}
A.~Crivellin and M.~Hoferichter,
%``Consequences of chirally enhanced explanations of (g \ensuremath{-} 2)$_{μ}$ for h \textrightarrow{} \ensuremath{\mu}\ensuremath{\mu} and Z \textrightarrow{} \ensuremath{\mu}\ensuremath{\mu},''
JHEP \textbf{07}, 135 (2021)
[erratum: JHEP \textbf{10}, 030 (2022)]
doi:10.1007/JHEP07(2021)135
[arXiv:2104.03202 [hep-ph]].
%84 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Capdevilla:2021rwo}
\bibitem{Capdevilla:2021rwo}
R.~Capdevilla, D.~Curtin, Y.~Kahn and G.~Krnjaic,
%``No-lose theorem for discovering the new physics of (g-2)\ensuremath{\mu} at muon colliders,''
Phys. Rev. D \textbf{105}, no.1, 015028 (2022)
doi:10.1103/PhysRevD.105.015028
[arXiv:2101.10334 [hep-ph]].
%92 citations counted in INSPIRE as of 16 Aug 2023

%\cite{Capdevilla:2020qel}
\bibitem{Capdevilla:2020qel}
R.~Capdevilla, D.~Curtin, Y.~Kahn and G.~Krnjaic,
%``Discovering the physics of $(g-2)_\mu$ at future muon colliders,''
Phys. Rev. D \textbf{103}, no.7, 075028 (2021)
doi:10.1103/PhysRevD.103.075028
[arXiv:2006.16277 [hep-ph]].
%92 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Khaw:2022qxh}
\bibitem{Khaw:2022qxh}
K.~S.~Khaw, Y.~Nakai, R.~Sato, Y.~Shigekami and Z.~Zhang,
%``A large muon EDM from dark matter,''
JHEP \textbf{02}, 234 (2023)
doi:10.1007/JHEP02(2023)234
[arXiv:2212.02891 [hep-ph]].
%0 citations counted in INSPIRE as of 18 Aug 2023

%\cite{Angelescu:2016mhl}
\bibitem{Angelescu:2016mhl}
A.~Angelescu and G.~Arcadi,
%``Dark Matter Phenomenology of SM and Enlarged Higgs Sectors Extended with Vector Like Leptons,''
Eur. Phys. J. C \textbf{77}, no.7, 456 (2017)
doi:10.1140/epjc/s10052-017-5015-2
[arXiv:1611.06186 [hep-ph]].
%18 citations counted in INSPIRE as of 21 Aug 2023

%\cite{Jana:2020joi}
\bibitem{Jana:2020joi}
S.~Jana, P.~K.~Vishnu, W.~Rodejohann and S.~Saad,
%``Dark matter assisted lepton anomalous magnetic moments and neutrino masses,''
Phys. Rev. D \textbf{102}, no.7, 075003 (2020)
doi:10.1103/PhysRevD.102.075003
[arXiv:2008.02377 [hep-ph]].
%63 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Arcadi:2021cwg}
\bibitem{Arcadi:2021cwg}
G.~Arcadi, L.~Calibbi, M.~Fedele and F.~Mescia,
%``Muon $g-2$ and $B$-anomalies from Dark Matter,''
Phys. Rev. Lett. \textbf{127}, no.6, 061802 (2021)
doi:10.1103/PhysRevLett.127.061802
[arXiv:2104.03228 [hep-ph]].
%70 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Frank:2021nkq}
\bibitem{Frank:2021nkq}
M.~Frank, Y.~Hi\c{c}y\i{}lmaz, S.~Mondal, \"O.~\"Ozdal and C.~S.~\"Un,
%``Electron and muon magnetic moments and implications for dark matter and model characterisation in non-universal U(1)' supersymmetric models,''
JHEP \textbf{10}, 063 (2021)
doi:10.1007/JHEP10(2021)063
[arXiv:2107.04116 [hep-ph]].
%24 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Athron:2021iuf}
\bibitem{Athron:2021iuf}
P.~Athron, C.~Bal\'azs, D.~H.~J.~Jacob, W.~Kotlarski, D.~St\"ockinger and H.~St\"ockinger-Kim,
%``New physics explanations of a$_{μ}$ in light of the FNAL muon g \ensuremath{-} 2 measurement,''
JHEP \textbf{09}, 080 (2021)
doi:10.1007/JHEP09(2021)080
[arXiv:2104.03691 [hep-ph]].
%204 citations counted in INSPIRE as of 18 Aug 2023

%\cite{Wojcik:2022woa}
\bibitem{Wojcik:2022woa}
G.~N.~Wojcik, L.~L.~Everett, S.~T.~Eu and R.~Ximenes,
%``Portal matter, kinetic mixing, and muon g \ensuremath{-} 2,''
Phys. Lett. B \textbf{841}, 137931 (2023)
doi:10.1016/j.physletb.2023.137931
[arXiv:2211.09918 [hep-ph]].
%4 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Endo:2020tkb}
\bibitem{Endo:2020tkb}
M.~Endo and S.~Mishima,
%``Muon $g − 2$ and CKM unitarity in extra lepton models,''
JHEP \textbf{08}, no.08, 004 (2020)
doi:10.1007/JHEP08(2020)004
[arXiv:2005.03933 [hep-ph]].
%41 citations counted in INSPIRE as of 21 Aug 2023

%\cite{Crivellin:2020ebi}
\bibitem{Crivellin:2020ebi}
A.~Crivellin, F.~Kirk, C.~A.~Manzari and M.~Montull,
%``Global Electroweak Fit and Vector-Like Leptons in Light of the Cabibbo Angle Anomaly,''
JHEP \textbf{12}, 166 (2020)
doi:10.1007/JHEP12(2020)166
[arXiv:2008.01113 [hep-ph]].
%87 citations counted in INSPIRE as of 21 Aug 2023

%\cite{Broggio:2014mna}
\bibitem{Broggio:2014mna}
A.~Broggio, E.~J.~Chun, M.~Passera, K.~M.~Patel and S.~K.~Vempati,
%``Limiting two-Higgs-doublet models,''
JHEP \textbf{11}, 058 (2014)
doi:10.1007/JHEP11(2014)058
[arXiv:1409.3199 [hep-ph]].
%168 citations counted in INSPIRE as of 26 Jul 2023

%\cite{Cherchiglia:2017uwv}
\bibitem{Cherchiglia:2017uwv}
A.~Cherchiglia, D.~St\"ockinger and H.~St\"ockinger-Kim,
%``Muon g-2 in the 2HDM: maximum results and detailed phenomenology,''
Phys. Rev. D \textbf{98}, 035001 (2018)
doi:10.1103/PhysRevD.98.035001
[arXiv:1711.11567 [hep-ph]].
%62 citations counted in INSPIRE as of 07 Aug 2023

%\cite{Athron:2021auq}
\bibitem{Athron:2021auq}
P.~Athron, C.~Balazs, T.~E.~Gonzalo, D.~Jacob, F.~Mahmoudi and C.~Sierra,
%``Likelihood analysis of the flavour anomalies and g \textendash{} 2 in the general two Higgs doublet model,''
JHEP \textbf{01}, 037 (2022)
doi:10.1007/JHEP01(2022)037
[arXiv:2111.10464 [hep-ph]].
%16 citations counted in INSPIRE as of 21 Aug 2023

%\cite{Nakai:2022vgp}
\bibitem{Nakai:2022vgp}
Y.~Nakai, R.~Sato and Y.~Shigekami,
%``Muon electric dipole moment as a probe of flavor-diagonal CP violation,''
Phys. Lett. B \textbf{831}, 137194 (2022)
doi:10.1016/j.physletb.2022.137194
[arXiv:2204.03183 [hep-ph]].
%3 citations counted in INSPIRE as of 01 Aug 2023

%\cite{Dermisek:2021ajd}
\bibitem{Dermisek:2021ajd}
R.~Dermisek, K.~Hermanek and N.~McGinnis,
%``Muon g-2 in two-Higgs-doublet models with vectorlike leptons,''
Phys. Rev. D \textbf{104}, no.5, 055033 (2021)
doi:10.1103/PhysRevD.104.055033
[arXiv:2103.05645 [hep-ph]].
%40 citations counted in INSPIRE as of 16 Aug 2023

%\cite{Dermisek:2020cod}
\bibitem{Dermisek:2020cod}
R.~Dermisek, K.~Hermanek, N.~McGinnis and N.~McGinnis,
%``Highly Enhanced Contributions of Heavy Higgs Bosons and New Leptons to Muon $g$\ensuremath{-}2 and Prospects at Future Colliders,''
Phys. Rev. Lett. \textbf{126}, no.19, 191801 (2021)
doi:10.1103/PhysRevLett.126.191801
[arXiv:2011.11812 [hep-ph]].
%26 citations counted in INSPIRE as of 16 Aug 2023

%\cite{Frank:2020smf}
\bibitem{Frank:2020smf}
M.~Frank and I.~Saha,
%``Muon anomalous magnetic moment in two-Higgs-doublet models with vectorlike leptons,''
Phys. Rev. D \textbf{102}, no.11, 115034 (2020)
doi:10.1103/PhysRevD.102.115034
[arXiv:2008.11909 [hep-ph]].
%31 citations counted in INSPIRE as of 16 Aug 2023

%\cite{Chun:2020uzw}
\bibitem{Chun:2020uzw}
E.~J.~Chun and T.~Mondal,
%``Explaining $g-2$ anomalies in two Higgs doublet model with vector-like leptons,''
JHEP \textbf{11}, 077 (2020)
doi:10.1007/JHEP11(2020)077
[arXiv:2009.08314 [hep-ph]].
%57 citations counted in INSPIRE as of 17 Aug 2023

%\cite{DelleRose:2020oaa}
\bibitem{DelleRose:2020oaa}
L.~Delle Rose, S.~Khalil and S.~Moretti,
%``Explaining electron and muon $g$ \ensuremath{-} 2 anomalies in an Aligned 2-Higgs Doublet Model with right-handed neutrinos,''
Phys. Lett. B \textbf{816}, 136216 (2021)
doi:10.1016/j.physletb.2021.136216
[arXiv:2012.06911 [hep-ph]].
%36 citations counted in INSPIRE as of 07 Aug 2023

%\cite{Ferreira:2021gke}
\bibitem{Ferreira:2021gke}
P.~M.~Ferreira, B.~L.~Gon\c{c}alves, F.~R.~Joaquim and M.~Sher,
%``(g-2)\ensuremath{\mu} in the 2HDM and slightly beyond: An updated view,''
Phys. Rev. D \textbf{104}, no.5, 053008 (2021)
doi:10.1103/PhysRevD.104.053008
[arXiv:2104.03367 [hep-ph]].
%33 citations counted in INSPIRE as of 01 Aug 2023

%\cite{Ghosh:2021jeg}
\bibitem{Ghosh:2021jeg}
N.~Ghosh and J.~Lahiri,
%``Generalized 2HDM with wrong-sign lepton-Yukawa coupling, in light of $g_{\mu }-2$ and lepton flavor violation at the future LHC,''
Eur. Phys. J. C \textbf{81}, no.12, 1074 (2021)
doi:10.1140/epjc/s10052-021-09844-9
[arXiv:2103.10632 [hep-ph]].
%14 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Han:2021gfu}
\bibitem{Han:2021gfu}
X.~F.~Han, T.~Li, H.~X.~Wang, L.~Wang and Y.~Zhang,
%``Lepton-specific inert two-Higgs-doublet model confronted with the new results for muon and electron g-2 anomalies and multilepton searches at the LHC,''
Phys. Rev. D \textbf{104}, no.11, 115001 (2021)
doi:10.1103/PhysRevD.104.115001
[arXiv:2104.03227 [hep-ph]].
%45 citations counted in INSPIRE as of 07 Aug 2023

%\cite{Dey:2021pyn}
\bibitem{Dey:2021pyn}
A.~Dey, J.~Lahiri and B.~Mukhopadhyaya,
%``Muon g-2 and a type-X two-Higgs-doublet scenario: Some studies in high-scale validity,''
Phys. Rev. D \textbf{106}, no.5, 055023 (2022)
doi:10.1103/PhysRevD.106.055023
[arXiv:2106.01449 [hep-ph]].
%17 citations counted in INSPIRE as of 07 Aug 2023

%\cite{Raju:2022zlv}
\bibitem{Raju:2022zlv}
M.~Raju, A.~Mukherjee and J.~P.~Saha,
%``Investigation of $(g-2)_{\mu }$ anomaly in the $\mu $-specific 2HDM with vector like leptons and the phenomenological implications,''
Eur. Phys. J. C \textbf{83}, no.5, 429 (2023)
doi:10.1140/epjc/s10052-023-11595-8
[arXiv:2207.02825 [hep-ph]].
%3 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Chakrabarty:2020jro}
\bibitem{Chakrabarty:2020jro}
N.~Chakrabarty,
%``Doubly charged scalars and vector-like leptons confronting the muon g-2 anomaly and Higgs vacuum stability,''
Eur. Phys. J. Plus \textbf{136}, no.11, 1183 (2021)
doi:10.1140/epjp/s13360-021-02168-3
[arXiv:2010.05215 [hep-ph]].
%15 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Chakrabarty:2021ztf}
\bibitem{Chakrabarty:2021ztf}
N.~Chakrabarty,
%``Muon g-2 in a type-X 2HDM assisted by inert scalars: A test at the LHC,''
Phys. Rev. D \textbf{107}, no.7, 075012 (2023)
doi:10.1103/PhysRevD.107.075012
[arXiv:2112.13126 [hep-ph]].
%2 citations counted in INSPIRE as of 01 Aug 2023

%\cite{Liu:2021kqp}
\bibitem{Liu:2021kqp}
G.~L.~Liu and P.~Zhou,
%``The Contribution of Charged Bosons with Right-Handed Neutrinos to the Muon g \ensuremath{-} 2 Anomaly in the Twin Higgs Models,''
Universe \textbf{8}, no.12, 654 (2022)
doi:10.3390/universe8120654
[arXiv:2101.00607 [hep-ph]].
%3 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Mondal:2021vou}
\bibitem{Mondal:2021vou}
T.~Mondal and H.~Okada,
%``Inverse seesaw and (g \ensuremath{-} 2) anomalies in B \ensuremath{-} L extended two Higgs doublet model,''
Nucl. Phys. B \textbf{976}, 115716 (2022)
doi:10.1016/j.nuclphysb.2022.115716
[arXiv:2103.13149 [hep-ph]].
%18 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Bharadwaj:2021tgp}
\bibitem{Bharadwaj:2021tgp}
H.~Bharadwaj, S.~Dutta and A.~Goyal,
%``Leptonic g \ensuremath{-} 2 anomaly in an extended Higgs sector with vector-like leptons,''
JHEP \textbf{11}, 056 (2021)
doi:10.1007/JHEP11(2021)056
[arXiv:2109.02586 [hep-ph]].
%19 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Lavoura:1994fv}
\bibitem{Lavoura:1994fv}
L.~Lavoura and J.~P.~Silva,
%``Fundamental CP violating quantities in a SU(2) x U(1) model with many Higgs doublets,''
Phys. Rev. D \textbf{50}, 4619-4624 (1994)
doi:10.1103/PhysRevD.50.4619
[arXiv:hep-ph/9404276 [hep-ph]].
%199 citations counted in INSPIRE as of 04 Aug 2023

%\cite{Lavoura:1994yu}
\bibitem{Lavoura:1994yu}
L.~Lavoura,
%``Signatures of discrete symmetries in the scalar sector,''
Phys. Rev. D \textbf{50}, 7089-7092 (1994)
doi:10.1103/PhysRevD.50.7089
[arXiv:hep-ph/9405307 [hep-ph]].
%42 citations counted in INSPIRE as of 25 Jul 2023

%\cite{Botella:1994cs}
\bibitem{Botella:1994cs}
F.~J.~Botella and J.~P.~Silva,
%``Jarlskog - like invariants for theories with scalars and fermions,''
Phys. Rev. D \textbf{51}, 3870-3875 (1995)
doi:10.1103/PhysRevD.51.3870
[arXiv:hep-ph/9411288 [hep-ph]].
%245 citations counted in INSPIRE as of 02 Aug 2023

%\cite{Davidson:2005cw}
\bibitem{Davidson:2005cw}
S.~Davidson and H.~E.~Haber,
%``Basis-independent methods for the two-Higgs-doublet model,''
Phys. Rev. D \textbf{72}, 035004 (2005)
[erratum: Phys. Rev. D \textbf{72}, 099902 (2005)]
doi:10.1103/PhysRevD.72.099902
[arXiv:hep-ph/0504050 [hep-ph]].
%458 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Crivellin:2020tsz}
\bibitem{Crivellin:2020tsz}
A.~Crivellin, D.~Mueller and F.~Saturnino,
%``Correlating h\textrightarrow{}\ensuremath{\mu}+\ensuremath{\mu}- to the Anomalous Magnetic Moment of the Muon via Leptoquarks,''
Phys. Rev. Lett. \textbf{127}, no.2, 021801 (2021)
doi:10.1103/PhysRevLett.127.021801
[arXiv:2008.02643 [hep-ph]].
%71 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Fajfer:2021cxa}
\bibitem{Fajfer:2021cxa}
S.~Fajfer, J.~F.~Kamenik and M.~Tammaro,
%``Interplay of New Physics effects in (g \ensuremath{-} 2)$_{ℓ}$ and h \textrightarrow{} \ensuremath{\ell}$^{+}$\ensuremath{\ell}$^{−}$ \textemdash{} lessons from SMEFT,''
JHEP \textbf{06}, 099 (2021)
doi:10.1007/JHEP06(2021)099
[arXiv:2103.10859 [hep-ph]].
%27 citations counted in INSPIRE as of 31 Jul 2023

%\cite{Dermisek:2021mhi}
\bibitem{Dermisek:2021mhi}
R.~Dermisek, K.~Hermanek and N.~McGinnis,
%``Di-Higgs and tri-Higgs boson signals of muon g-2 at a muon collider,''
Phys. Rev. D \textbf{104}, no.9, L091301 (2021)
doi:10.1103/PhysRevD.104.L091301
[arXiv:2108.10950 [hep-ph]].
%24 citations counted in INSPIRE as of 16 Aug 2023

%\cite{Dermisek:2022aec}
\bibitem{Dermisek:2022aec}
R.~Dermisek, K.~Hermanek, N.~McGinnis and S.~Yoon,
%``Ellipse of Muon Dipole Moments,''
Phys. Rev. Lett. \textbf{129}, no.22, 221801 (2022)
doi:10.1103/PhysRevLett.129.221801
[arXiv:2205.14243 [hep-ph]].
%9 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Dermisek:2023nhe}
\bibitem{Dermisek:2023nhe}
R.~Dermisek, K.~Hermanek, N.~McGinnis and S.~Yoon,
%``Effective field theory of chirally enhanced muon mass and dipole operators,''
Phys. Rev. D \textbf{107}, no.9, 095043 (2023)
doi:10.1103/PhysRevD.107.095043
[arXiv:2302.14144 [hep-ph]].
%2 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Crivellin:2022wzw}
\bibitem{Crivellin:2022wzw}
A.~Crivellin and M.~Hoferichter,
%``The Anomalous Magnetic Moment of the Muon: Beyond the Standard Model via Chiral Enhancement,''
[arXiv:2207.01912 [hep-ph]].
%4 citations counted in INSPIRE as of 07 Aug 2023

%\cite{Hamaguchi:2022byw}
\bibitem{Hamaguchi:2022byw}
K.~Hamaguchi, N.~Nagata, G.~Osaki and S.~Y.~Tseng,
%``Probing new physics in the vector-like lepton model by lepton electric dipole moments,''
JHEP \textbf{01}, 100 (2023)
doi:10.1007/JHEP01(2023)100
[arXiv:2211.16800 [hep-ph]].
%4 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Dermisek:2015oja}
\bibitem{Dermisek:2015oja}
R.~Dermisek, E.~Lunghi and S.~Shin,
%``Two Higgs doublet model with vectorlike leptons and contributions to $pp\to WW$ and $H\to WW$,''
JHEP \textbf{02}, 119 (2016)
doi:10.1007/JHEP02(2016)119
[arXiv:1509.04292 [hep-ph]].
%37 citations counted in INSPIRE as of 16 Aug 2023

%\cite{Gunion:2002zf}
\bibitem{Gunion:2002zf}
J.~F.~Gunion and H.~E.~Haber,
%``The CP conserving two Higgs doublet model: The Approach to the decoupling limit,''
Phys. Rev. D \textbf{67}, 075019 (2003)
doi:10.1103/PhysRevD.67.075019
[arXiv:hep-ph/0207010 [hep-ph]].
%955 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Lee:1977eg}
\bibitem{Lee:1977eg}
B.~W.~Lee, C.~Quigg and H.~B.~Thacker,
%``Weak Interactions at Very High-Energies: The Role of the Higgs Boson Mass,''
Phys. Rev. D \textbf{16}, 1519 (1977)
doi:10.1103/PhysRevD.16.1519
%2388 citations counted in INSPIRE as of 22 Aug 2023

%\cite{Lee:1977yc}
\bibitem{Lee:1977yc}
B.~W.~Lee, C.~Quigg and H.~B.~Thacker,
%``The Strength of Weak Interactions at Very High-Energies and the Higgs Boson Mass,''
Phys. Rev. Lett. \textbf{38}, 883-885 (1977)
doi:10.1103/PhysRevLett.38.883
%872 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Cornwall:1974km}
\bibitem{Cornwall:1974km}
J.~M.~Cornwall, D.~N.~Levin and G.~Tiktopoulos,
%``Derivation of Gauge Invariance from High-Energy Unitarity Bounds on the s Matrix,''
Phys. Rev. D \textbf{10}, 1145 (1974)
[erratum: Phys. Rev. D \textbf{11}, 972 (1975)]
doi:10.1103/PhysRevD.10.1145
%1357 citations counted in INSPIRE as of 04 Aug 2023

%\cite{Ginzburg:2005dt}
\bibitem{Ginzburg:2005dt}
I.~F.~Ginzburg and I.~P.~Ivanov,
%``Tree-level unitarity constraints in the most general 2HDM,''
Phys. Rev. D \textbf{72}, 115010 (2005)
doi:10.1103/PhysRevD.72.115010
[arXiv:hep-ph/0508020 [hep-ph]].
%299 citations counted in INSPIRE as of 04 Aug 2023

%\cite{Kanemura:2015ska}
\bibitem{Kanemura:2015ska}
S.~Kanemura and K.~Yagyu,
%``Unitarity bound in the most general two Higgs doublet model,''
Phys. Lett. B \textbf{751}, 289-296 (2015)
doi:10.1016/j.physletb.2015.10.047
[arXiv:1509.06060 [hep-ph]].
%105 citations counted in INSPIRE as of 07 Aug 2023

%\cite{Jurciukonis:2018skr}
\bibitem{Jurciukonis:2018skr}
D.~Jur\v{c}iukonis and L.~Lavoura,
%``The three- and four-Higgs couplings in the general two-Higgs-doublet model,''
JHEP \textbf{12}, 004 (2018)
doi:10.1007/JHEP12(2018)004
[arXiv:1807.04244 [hep-ph]].
%16 citations counted in INSPIRE as of 18 Jul 2023

%\cite{Marciano:1989ns}
\bibitem{Marciano:1989ns}
W.~J.~Marciano, G.~Valencia and S.~Willenbrock,
%``Renormalization Group Improved Unitarity Bounds on the Higgs Boson and Top Quark Masses,''
Phys. Rev. D \textbf{40}, 1725 (1989)
doi:10.1103/PhysRevD.40.1725
%169 citations counted in INSPIRE as of 26 Jun 2023

%\cite{Maalampi:1991fb}
\bibitem{Maalampi:1991fb}
J.~Maalampi, J.~Sirkka and I.~Vilja,
%``Tree level unitarity and triviality bounds for two Higgs models,''
Phys. Lett. B \textbf{265}, 371-376 (1991)
doi:10.1016/0370-2693(91)90068-2
%110 citations counted in INSPIRE as of 26 Jun 2023

%\cite{Kanemura:1993hm}
\bibitem{Kanemura:1993hm}
S.~Kanemura, T.~Kubota and E.~Takasugi,
%``Lee-Quigg-Thacker bounds for Higgs boson masses in a two doublet model,''
Phys. Lett. B \textbf{313}, 155-160 (1993)
doi:10.1016/0370-2693(93)91205-2
[arXiv:hep-ph/9303263 [hep-ph]].
%425 citations counted in INSPIRE as of 09 Aug 2023

%\cite{ATLAS:2020zms}
\bibitem{ATLAS:2020zms}
G.~Aad \textit{et al.} [ATLAS],
%``Search for heavy Higgs bosons decaying into two tau leptons with the ATLAS detector using $pp$ collisions at $\sqrt{s}=13$ TeV,''
Phys. Rev. Lett. \textbf{125}, no.5, 051801 (2020)
doi:10.1103/PhysRevLett.125.051801
[arXiv:2002.12223 [hep-ex]].
%245 citations counted in INSPIRE as of 17 Aug 2023

%\cite{ATLAS:2021upq}
\bibitem{ATLAS:2021upq}
G.~Aad \textit{et al.} [ATLAS],
%``Search for charged Higgs bosons decaying into a top quark and a bottom quark at $ \sqrt{\mathrm{s}} $ = 13 TeV with the ATLAS detector,''
JHEP \textbf{06}, 145 (2021)
doi:10.1007/JHEP06(2021)145
[arXiv:2102.10076 [hep-ex]].
%111 citations counted in INSPIRE as of 14 Aug 2023

%\cite{Guedes:2022cfy}
\bibitem{Guedes:2022cfy}
G.~Guedes and P.~Olgoso,
%``A bridge to new physics: proposing new \textemdash{} and reviving old \textemdash{} explanations of a$_{μ}$,''
JHEP \textbf{09}, 181 (2022)
doi:10.1007/JHEP09(2022)181
[arXiv:2205.04480 [hep-ph]].
%15 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Freitas:2014pua}
\bibitem{Freitas:2014pua}
A.~Freitas, J.~Lykken, S.~Kell and S.~Westhoff,
%``Testing the Muon g-2 Anomaly at the LHC,''
JHEP \textbf{05}, 145 (2014)
[erratum: JHEP \textbf{09}, 155 (2014)]
doi:10.1007/JHEP09(2014)155
[arXiv:1402.7065 [hep-ph]].
%105 citations counted in INSPIRE as of 21 Aug 2023

%\cite{Muong-2:2008ebm}
\bibitem{Muong-2:2008ebm}
G.~W.~Bennett \textit{et al.} [Muon (g-2)],
%``An Improved Limit on the Muon Electric Dipole Moment,''
Phys. Rev. D \textbf{80}, 052008 (2009)
doi:10.1103/PhysRevD.80.052008
[arXiv:0811.1207 [hep-ex]].
%357 citations counted in INSPIRE as of 14 Aug 2023

%\cite{Lukicov:2019ibv}
\bibitem{Lukicov:2019ibv}
G.~Lukicov [Muon g-2],
%``The Fermilab Muon $g-2$ Straw Tracking Detectors, Internal Tracker Alignment, and the Muon EDM Measurement,''
[arXiv:1909.12900 [physics.ins-det]].
%3 citations counted in INSPIRE as of 27 Jul 2023

%\cite{Adelmann:2021udj}
\bibitem{Adelmann:2021udj}
A.~Adelmann, M.~Backhaus, C.~Chavez Barajas, N.~Berger, T.~Bowcock, C.~Calzolaio, G.~Cavoto, R.~Chislett, A.~Crivellin and M.~Daum, \textit{et al.}
%``Search for a muon EDM using the frozen-spin technique,''
[arXiv:2102.08838 [hep-ex]].
%41 citations counted in INSPIRE as of 17 Aug 2023

%\cite{CMS:2019hsm}
\bibitem{CMS:2019hsm}
A.~M.~Sirunyan \textit{et al.} [CMS],
%``Search for vector-like leptons in multilepton final states in proton-proton collisions at $\sqrt{s}$ = 13 TeV,''
Phys. Rev. D \textbf{100}, no.5, 052003 (2019)
doi:10.1103/PhysRevD.100.052003
[arXiv:1905.10853 [hep-ex]].
%85 citations counted in INSPIRE as of 17 Aug 2023

%\cite{ATLAS:2022yhd}
\bibitem{ATLAS:2022yhd}
G.~Aad \textit{et al.} [ATLAS],
%``Search for type-III seesaw heavy leptons in leptonic final states in pp collisions at $\sqrt{s} = 13~\text {TeV}$ with the ATLAS detector,''
Eur. Phys. J. C \textbf{82}, no.11, 988 (2022)
doi:10.1140/epjc/s10052-022-10785-0
[arXiv:2202.02039 [hep-ex]].
%19 citations counted in INSPIRE as of 16 Aug 2023

%\cite{ATLAS:2015qoy}
\bibitem{ATLAS:2015qoy}
G.~Aad \textit{et al.} [ATLAS],
%``Search for heavy lepton resonances decaying to a $Z$ boson and a lepton in $pp$ collisions at $\sqrt{s}=8$ TeV with the ATLAS detector,''
JHEP \textbf{09}, 108 (2015)
doi:10.1007/JHEP09(2015)108
[arXiv:1506.01291 [hep-ex]].
%104 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Buttazzo:2020ibd}
\bibitem{Buttazzo:2020ibd}
D.~Buttazzo and P.~Paradisi,
%``Probing the muon $g-2$ anomaly with the Higgs boson at a muon collider,''
Phys. Rev. D \textbf{104}, no.7, 075021 (2021)
doi:10.1103/PhysRevD.104.075021
[arXiv:2012.02769 [hep-ph]].
%79 citations counted in INSPIRE as of 21 Aug 2023

%\cite{Han:2020pif}
\bibitem{Han:2020pif}
T.~Han, D.~Liu, I.~Low and X.~Wang,
%``Electroweak couplings of the Higgs boson at a multi-TeV muon collider,''
Phys. Rev. D \textbf{103}, no.1, 013002 (2021)
doi:10.1103/PhysRevD.103.013002
[arXiv:2008.12204 [hep-ph]].
%80 citations counted in INSPIRE as of 16 Aug 2023

%\cite{Han:2021lnp}
\bibitem{Han:2021lnp}
T.~Han, W.~Kilian, N.~Kreher, Y.~Ma, J.~Reuter, T.~Striegl and K.~Xie,
%``Precision test of the muon-Higgs coupling at a high-energy muon collider,''
JHEP \textbf{12}, 162 (2021)
doi:10.1007/JHEP12(2021)162
[arXiv:2108.05362 [hep-ph]].
%29 citations counted in INSPIRE as of 08 Aug 2023

%\cite{deBlas:2022aow}
\bibitem{deBlas:2022aow}
J.~de Blas, J.~Gu and Z.~Liu,
%``Higgs boson precision measurements at a 125~GeV muon collider,''
Phys. Rev. D \textbf{106}, no.7, 073007 (2022)
doi:10.1103/PhysRevD.106.073007
[arXiv:2203.04324 [hep-ph]].
%17 citations counted in INSPIRE as of 17 Aug 2023

%\cite{Forslund:2022xjq}
\bibitem{Forslund:2022xjq}
M.~Forslund and P.~Meade,
%``High precision higgs from high energy muon colliders,''
JHEP \textbf{08}, 185 (2022)
doi:10.1007/JHEP08(2022)185
[arXiv:2203.09425 [hep-ph]].
%19 citations counted in INSPIRE as of 16 Aug 2023

%\cite{Arakawa:2022mkr}
\bibitem{Arakawa:2022mkr}
J.~Arakawa, A.~Rajaraman, T.~Sui and T.~M.~P.~Tait,
%``Probing Muon $g-2$ at a Future Muon Collider,''
[arXiv:2208.14464 [hep-ph]].
%5 citations counted in INSPIRE as of 01 Aug 2023

%\cite{Nie:1998yn}
\bibitem{Nie:1998yn}
S.~Nie and M.~Sher,
%``Vacuum stability bounds in the two Higgs doublet model,''
Phys. Lett. B \textbf{449}, 89-92 (1999)
doi:10.1016/S0370-2693(99)00019-2
[arXiv:hep-ph/9811234 [hep-ph]].
%187 citations counted in INSPIRE as of 11 Aug 2023

%\cite{Deshpande:1977rw}
\bibitem{Deshpande:1977rw}
N.~G.~Deshpande and E.~Ma,
%``Pattern of Symmetry Breaking with Two Higgs Doublets,''
Phys. Rev. D \textbf{18}, 2574 (1978)
doi:10.1103/PhysRevD.18.2574
%917 citations counted in INSPIRE as of 09 Aug 2023

%\cite{Barroso:2013awa}
\bibitem{Barroso:2013awa}
A.~Barroso, P.~M.~Ferreira, I.~P.~Ivanov and R.~Santos,
%``Metastability bounds on the two Higgs doublet model,''
JHEP \textbf{06}, 045 (2013)
doi:10.1007/JHEP06(2013)045
[arXiv:1303.5098 [hep-ph]].
%179 citations counted in INSPIRE as of 09 Aug 2023
